Iterative Refinement Graph Neural Network for Antibody Sequence-Structure Co-design

Antibodies are versatile proteins that bind to pathogens like viruses and stimulate the adaptive immune system. The specificity of antibody binding is determined by complementarity-determining regions (CDRs) at the tips of these Y-shaped proteins. In this paper, we propose a generative model to automatically design the CDRs of antibodies with enhanced binding specificity or neutralization capabilities. Previous generative approaches formulate protein design as a structure-conditioned sequence generation task, assuming the desired 3D structure is given a priori. In contrast, we propose to co-design the sequence and 3D structure of CDRs as graphs. Our model unravels a sequence autoregressively while iteratively refining its predicted global structure. The inferred structure in turn guides subsequent residue choices. For efficiency, we model the conditional dependence between residues inside and outside of a CDR in a coarse-grained manner. Our method achieves superior log-likelihood on the test set and outperforms previous baselines in designing antibodies capable of neutralizing the SARS-CoV-2 virus.

==> jeremy_intro.tex <==
\section{Introduction}

Monoclonal antibodies are increasingly adopted as therapeutics targeting a wide range of pathogens such as SARS-CoV2~\citep{pinto2020cross}. Since the binding specificity of these Y-shaped proteins is largely determined by the complementarity determining regions (CDRs) at their tips, the main goal for computational antibody design is to automate the creation of CDR subsequences with desired properties. This problem is particularly challenging due to the combinatorial search space of over $20^{20}$ possible amino acid sequences and small solution space shaped by multiple constraints including binding affinity, stability, and developability \citep{raybould2019five}.

One of the key design question in CDR generation is the relation between the sequence and the underlying 3D structure. Generating sequences without the corresponding structure can lead to sub-optimal performance \citep{alley2019unified,shin2021protein} while generating from a pre-defined 3D structure ~\citep{ingraham2019generative,karimi2020novo} restricts the diversity and novelty of designs~\citep{cao2021fold2seq} since the optimal structure for neutralization or binding is often unknown, especially for new pathogens. Therefore, it is crucial to develop generative models for sequence and structure co-design. 

Another important design consideration is the ability for the model to optimize for various properties such as neutralization or binding to multiple targets. While traditional physics-based methods \citep{pantazes2010optcdr,li2014optmaven,lapidoth2015abdesign,adolf2018rosettaantibodydesign} can use energy function minimization to co-design an antibody sequence and its structure, they only allow to optimize for binding affinity, which limits their applicability.

In this paper, we propose to represent an antibody sequence and structure as a graph and formulate the co-design task as a graph generation problem. Most of prior models for graph generation~\citep{liu2018constrained,gebauer2019symmetry} predict nodes and edges autoregressively. As a result, they cannot \emph{revise} the generated subgraph when new nodes are added. Allowing graph revision is crucial to our co-design task because an antibody structure is expected to change as new nodes are inserted.

Given this motivation, we propose a novel iterative refinement architecture for graph generation. Our model unravels a sequence autoregressively while revising its associated structure by repredicting pairwise distance and angles between all nodes. We then encode a revised graph structure using a message passing network to guide subsequent amino acid choices. Since our model only generates the CDR of an antibody with the framework region fixed, we propose to coarsen the subgraph outside of the CDR's for computational efficiency. After pretraining our model on antibodies with known structures, we finetune it using a predefined property predictor to generate antibodies with specific properties.

We evaluate our method on three antibody generation tasks, ranging from SARS-CoV-2 neutralization optimization to antigen-binding antibody design. We compare our model a standard unconditional sequence model~\citep{hochreiter1997long} and a state-of-the-art method for graph generation~\citep{gebauer2019symmetry}. Our method not only achieves lower perplexity on test sequences but also outperforms previous baselines in property-guided antibody design tasks.

\begin{table}[t]
\centering
\caption{SARS-CoV-2 neutralization optimization results. \textit{Left}: We report the avearge improvement metric of different methods. \textit{Right}: Examples of new CDR-H3 sequences generated by our model and their predicted neutralization improvement over original antibodies S1D7 and C694.}
\label{tab:covid}
\begin{subtable}{0.35\textwidth}
\begin{tabular}{lc}
\hline
Model & Improvement \Tstrut\Bstrut \\
\hline
LSTM & 10.1\% \Tstrut\Bstrut\\
AR-GNN & 9.3\% \Tstrut\Bstrut\\
\hline
RefineGNN & \textbf{11.7\%} \Tstrut\Bstrut\\
\hline
\end{tabular}
\end{subtable}
~
\begin{subtable}{0.63\textwidth}
\begin{tabular}{lcc}
\hline
Antibody: & S1D7 & C694   \Tstrut\Bstrut \\
\hline
Old CDR-H3 & \texttt{TRGHSDY} & \texttt{ARDRGYDSSGPDAFDI}  \Tstrut\Bstrut\\
New CDR-H3 & \texttt{ARWWMDV} & \texttt{ARERIIIVSISAWMDV} \Tstrut\Bstrut\\
Improvement & 63\% $\rightarrow$ 73\% & 82\% $\rightarrow$ 91\% \Tstrut\Bstrut\\
\hline
\end{tabular}
\end{subtable}
\end{table}


\textbf{Results.} All methods are pretrained on SAbDab antibodies and finetuned on CoVAbDab using the ITA algorithm to generate neutralizing antibodies. Our model outperforms the best baseline by a 8\% increase in average neutralization score (Table~\ref{tab:covid}). Our pretrained RefineGNN also achieves a much lower perplexity on CoVAbDab antibodies. 
To understand the tradeoff between the perplexity constraint and neutralization improvement, we also report model performance with a looser PPL cutoff at 10. Our model still outperforms other methods, but with a smaller margin. This shows that our model is better at generating realistic CDR sequences than other methods.
%Examples of generated CDR-H3 sequences and their predicted neutralization scores are shown in the appendix.

\begin{table}[t]
\centering
\caption{SARS-CoV-2 neutralization optimization results. For each method, we report their PPL on CoVAbDab CDR-H3 sequences before ITA finetuning and their average neutralization score after ITA finetuning. The average neutralization probability of original CoVAbDab antibodies is 69.3\%. }
\vspace{-4pt}
\label{tab:covid}
\begin{tabular}{lcccc}
\hline
     & Original & LSTM & AR-GNN & RefineGNN \Tstrut\Bstrut \\
    \hline
    CoVAbDab PPL & - & 9.40 & 8.67 & \textbf{7.86} \Tstrut\Bstrut \\
    Neutralization (PPL cutoff=8) & 69.3\% & 71.6\% & 71.8\% & \textbf{80.5\%} \Tstrut\Bstrut \\
    Neutralization (PPL cutoff=10) & 69.3\% & 79.4\% & 78.6\% & \textbf{81.0\%} \Tstrut\Bstrut \\
\hline
\end{tabular}

\end{table}
